The Optical Green Valley vs Mid-IR Canyon in Compact Groups

Compact groups of galaxies provide conditions similar to those experienced by galaxies in the earlier universe. Recent work on compact groups has led to the discovery of a dearth of mid-infrared transition galaxies (MIRTGs) in IRAC (3.6 - 8.0 micron) color space (Johnson et al. 2007; Walker et al. 2012) as well as at intermediate specific star formation rates (Tzanavaris et al. 2010). However, we find that in compact groups these mid-infrared (mid-IR) transition galaxies in the mid-infrared dearth have already transitioned to the optical ([g-r]) red sequence. We investigate the optical color-magnitude diagram (CMD) of 99 compact groups containing 348 galaxies and compare the optical CMD with mid-IR color space for compact group galaxies. Utilizing redshifts available from SDSS, we identified new galaxy members for 6 groups. By combining optical and mid-IR data, we obtain information on both the dust and the stellar populations in compact group galaxies. We also compare with more isolated galaxies and galaxies in the Coma cluster, which reveals that, similar to clusters, compact groups are dominated by optically red galaxies. While we find that compact group transition galaxies lie on the optical red sequence, LVL+SINGS mid-IR transition galaxies span the range of optical colors. The dearth of mid-IR transition galaxies in compact groups may be due to a lack of moderately star forming low mass galaxies; the relative lack of these galaxies could be due to their relatively small gravitational potential wells. This makes them more susceptible to this dynamic environment, thus causing them to more easily lose gas or be accreted by larger members.

==> cangals.tex <==
\ProvidesFile{cangals.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{cccccc}
\tablewidth{0pt}
\tablecaption{Galaxies in the \mir Canyon\label{cangals}}
\tablehead{
\colhead{Galaxy} &	\colhead{R.A.\tablenotemark{a}} &	\colhead{Dec\tablenotemark{a}} &	\colhead{D\tablenotemark{a}} &	\colhead{Morphology\tablenotemark{a}} &	\colhead{$g-r$} \\
\colhead{} &	\colhead{(J2000)} &	\colhead{(J2000)} &	\colhead{(Mpc)} &	\colhead{} &	\colhead{mag}}
\startdata
H37e & 09$^\mathrm{h}$13$^\mathrm{m}$34\fs0 & +30\degr02\arcmin23\arcsec & 92.6 & E0 & 0.75\\
H57b & 11$^\mathrm{h}$37$^\mathrm{m}$43\fs6 & +22\degr00\arcmin35\arcsec & 130.5 & SBb & 0.74\\
H57h & 11$^\mathrm{h}$37$^\mathrm{m}$50\fs5 & +22\degr00\arcmin45\arcsec & 133.5 & SBb & 0.75\\
H79b & 15$^\mathrm{h}$59$^\mathrm{m}$12\fs5 & +20\degr45\arcmin48\arcsec & 69.4 & S0pec & 0.72
\enddata
\tablenotetext{a}{Galaxy RA, Dec, distance (corrected for Virgo+GA+Shapley), and morphology taken from NED. The cosmology used was $H_0=73\;{\rm km\,s^{-1}\,Mpc^{-1}}$, $\Omega_{matter}=0.27$, and $\Omega_{vacuum}=0.73$.}
\end{deluxetable}

\endinput
%%
%% End of file `cangals.tex'.


==> hcggals.tex <==
\ProvidesFile{hcggals.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{cccc}
\tabletypesize{\small}
\tablewidth{0pt}
\tablecolumns{4}
\tablecaption{Photometry for HCG Galaxies\label{hcggals}}
\tablehead{
\colhead{Galaxy} &	\colhead{g'} &	\colhead{r'} &	\colhead{i'} \\
\colhead{} &	\colhead{mag} &	\colhead{mag} &	\colhead{mag}
}
\startdata
\sidehead{HCG 1}
A & $14.95 \pm 0.02$ & $14.38 \pm 0.01$ & $14.11 \pm 0.01$ \\
B & $15.16 \pm 0.02$ & $14.52 \pm 0.01$ & $14.24 \pm 0.01$ \\
C & $16.53 \pm 0.01$ & $15.80 \pm 0.01$ & $15.44 \pm 0.02$ \\
D & $15.32 \pm 0.01$ & $14.50 \pm 0.01$ & $14.14 \pm 0.01$ \\
\sidehead{HCG 2}
A & $13.55 \pm 0.01$ & $13.24 \pm 0.01$ & $13.17 \pm 0.01$ \\
B & $14.07 \pm 0.01$ & $13.58 \pm 0.01$ & $13.43 \pm 0.01$ \\
C & $14.51 \pm 0.01$ & $14.05 \pm 0.01$ & $13.87 \pm 0.01$ \\
\sidehead{HCG 3}
A & $14.87 \pm 0.01$ & $14.23 \pm 0.01$ & $13.94 \pm 0.01$ \\
B & $14.97 \pm 0.01$ & $14.15 \pm 0.01$ & $13.78 \pm 0.01$ \\
D & $15.18 \pm 0.01$ & $14.39 \pm 0.01$ & $14.03 \pm 0.01$ \\
\sidehead{HCG 4}
A & $13.35 \pm 0.01$ & $12.86 \pm 0.01$ & $12.67 \pm 0.01$ \\
B & $15.20 \pm 0.01$ & $14.70 \pm 0.01$ & $14.53 \pm 0.01$ \\
C & $15.50 \pm 0.01$ & $14.69 \pm 0.01$ & $14.35 \pm 0.01$ \\
D & $15.57 \pm 0.01$ & $14.96 \pm 0.01$ & $14.71 \pm 0.01$ \\
\sidehead{HCG 7\tablenotemark{a}}
A & $13.03 \pm 0.01$ & $12.27 \pm 0.01$ & $11.95 \pm 0.01$ \\
B & $13.77 \pm 0.01$ & $13.00 \pm 0.01$ & $12.64 \pm 0.01$ \\
C & $13.24 \pm 0.01$ & $12.65 \pm 0.01$ & $12.47 \pm 0.01$ \\
D & $14.96 \pm 0.01$ & $14.41 \pm 0.01$ & $14.16 \pm 0.01$ \\
\sidehead{HCG 10\tablenotemark{b}}
A & $12.97 \pm 0.01$ & $12.18 \pm 0.01$ & $11.78 \pm 0.01$ \\
B & $12.88 \pm 0.01$ & $12.09 \pm 0.01$ & $11.71 \pm 0.01$ \\
C & $14.25 \pm 0.01$ & $13.43 \pm 0.01$ & $13.03 \pm 0.01$ \\
D & $15.12 \pm 0.01$ & $14.42 \pm 0.01$ & $14.09 \pm 0.01$ \\
\sidehead{HCG 14}
A & $14.48 \pm 0.01$ & $13.70 \pm 0.01$ & $13.34 \pm 0.01$ \\
B & $14.08 \pm 0.01$ & $13.33 \pm 0.01$ & $13.00 \pm 0.01$ \\
C & $15.68 \pm 0.01$ & $14.95 \pm 0.01$ & $14.67 \pm 0.01$ \\
\sidehead{HCG 15}
A & $14.13 \pm 0.01$ & $13.31 \pm 0.01$ & $12.91 \pm 0.01$ \\
B & $14.25 \pm 0.01$ & $13.48 \pm 0.01$ & $13.13 \pm 0.01$ \\
C & $14.25 \pm 0.01$ & $13.47 \pm 0.01$ & $13.11 \pm 0.01$ \\
D & $14.59 \pm 0.01$ & $13.84 \pm 0.01$ & $13.49 \pm 0.01$ \\
E & $14.90 \pm 0.01$ & $14.15 \pm 0.01$ & $13.82 \pm 0.01$ \\
F & $15.85 \pm 0.01$ & $15.32 \pm 0.01$ & $15.09 \pm 0.02$ \\
\sidehead{HCG 16\tablenotemark{c}}
A & $12.54 \pm 0.01$ & $11.83 \pm 0.01$ & $11.49 \pm 0.01$ \\
B & $13.26 \pm 0.01$ & $12.44 \pm 0.01$ & $12.05 \pm 0.01$ \\
C & $13.20 \pm 0.01$ & $12.57 \pm 0.01$ & $12.34 \pm 0.01$ \\
\sidehead{HCG 22\tablenotemark{d}}
A & $12.30 \pm 0.01$ & $11.50 \pm 0.01$ & $11.11 \pm 0.01$ \\
B & $14.60 \pm 0.01$ & $13.91 \pm 0.01$ & $13.58 \pm 0.01$ \\
C & $13.79 \pm 0.01$ & $13.26 \pm 0.01$ & $13.04 \pm 0.01$ \\
\sidehead{HCG 25}
A & $14.10 \pm 0.01$ & $13.70 \pm 0.01$ & $13.55 \pm 0.01$ \\
B & $14.10 \pm 0.02$ & $13.30 \pm 0.01$ & $12.91 \pm 0.01$ \\
D & $15.53 \pm 0.01$ & $14.88 \pm 0.01$ & $14.61 \pm 0.01$ \\
F & $15.88 \pm 0.02$ & $15.15 \pm 0.01$ & $14.84 \pm 0.01$ \\
\sidehead{HCG 31}
AC & $13.52 \pm 0.01$ & $13.28 \pm 0.01$ & $13.32 \pm 0.01$ \\
B & $15.17 \pm 0.01$ & $14.96 \pm 0.01$ & $14.94 \pm 0.01$ \\
E & $17.15 \pm 0.02$ & $17.00 \pm 0.02$ & $17.18 \pm 0.02$ \\
F & $17.25 \pm 0.02$ & $17.40 \pm 0.02$ & $17.41 \pm 0.03$ \\
G & $14.59 \pm 0.01$ & $14.38 \pm 0.01$ & $14.35 \pm 0.01$ \\
Q & $16.48 \pm 0.01$ & $16.18 \pm 0.01$ & $16.08 \pm 0.01$ \\
\sidehead{HCG 37}
A & $12.96 \pm 0.01$ & $12.20 \pm 0.01$ & $11.85 \pm 0.01$ \\
B & $14.52 \pm 0.01$ & $13.69 \pm 0.01$ & $13.30 \pm 0.01$ \\
C & $15.71 \pm 0.03$ & $14.95 \pm 0.03$ & $14.61 \pm 0.03$ \\
D & $16.39 \pm 0.01$ & $15.86 \pm 0.01$ & $15.66 \pm 0.01$ \\
E & $16.40 \pm 0.01$ & $15.64 \pm 0.01$ & $15.31 \pm 0.01$ \\
\sidehead{HCG 38}
A & $15.40 \pm 0.01$ & $14.60 \pm 0.01$ & $14.22 \pm 0.01$ \\
B & $14.67 \pm 0.01$ & $14.02 \pm 0.01$ & $13.70 \pm 0.01$ \\
C & $15.76 \pm 0.02$ & $15.05 \pm 0.02$ & $14.73 \pm 0.01$ \\
\sidehead{HCG 43}
A & $15.36 \pm 0.01$ & $14.63 \pm 0.01$ & $14.30 \pm 0.01$ \\
B & $15.76 \pm 0.01$ & $15.16 \pm 0.01$ & $14.90 \pm 0.01$ \\
C & $15.52 \pm 0.01$ & $14.73 \pm 0.01$ & $14.38 \pm 0.01$ \\
D & $16.71 \pm 0.01$ & $16.05 \pm 0.01$ & $15.77 \pm 0.01$ \\
E & $16.80 \pm 0.01$ & $15.92 \pm 0.01$ & $15.54 \pm 0.01$ \\
\sidehead{HCG 44\tablenotemark{e}}
A & $11.34 \pm 0.01$ & $10.57 \pm 0.01$ & $10.16 \pm 0.01$ \\
B & $11.49 \pm 0.01$ & $10.74 \pm 0.01$ & $10.35 \pm 0.01$ \\
C & $12.60 \pm 0.01$ & $11.91 \pm 0.01$ & $11.56 \pm 0.01$ \\
D & $13.40 \pm 0.01$ & $12.97 \pm 0.01$ & $12.82 \pm 0.01$ \\
\sidehead{HCG 46}
A & $15.48 \pm 0.01$ & $14.68 \pm 0.01$ & $14.32 \pm 0.01$ \\
B & $15.49 \pm 0.01$ & $14.72 \pm 0.01$ & $14.34 \pm 0.01$ \\
C & $15.47 \pm 0.01$ & $14.68 \pm 0.01$ & $14.32 \pm 0.01$ \\
D & $15.69 \pm 0.01$ & $14.90 \pm 0.01$ & $14.56 \pm 0.01$ \\
\sidehead{HCG 47}
A & $14.10 \pm 0.01$ & $13.42 \pm 0.01$ & $13.11 \pm 0.01$ \\
B & $14.97 \pm 0.01$ & $14.15 \pm 0.01$ & $13.78 \pm 0.01$ \\
C & $16.22 \pm 0.01$ & $15.54 \pm 0.01$ & $15.27 \pm 0.01$ \\
D & $15.79 \pm 0.01$ & $15.14 \pm 0.01$ & $14.87 \pm 0.01$ \\
\sidehead{HCG 49}
A & $15.91 \pm 0.01$ & $15.59 \pm 0.01$ & $15.50 \pm 0.01$ \\
B & $16.42 \pm 0.01$ & $16.28 \pm 0.01$ & $16.28 \pm 0.01$ \\
C & $17.25 \pm 0.01$ & $16.99 \pm 0.01$ & $16.96 \pm 0.01$ \\
D & $17.00 \pm 0.01$ & $16.72 \pm 0.01$ & $16.67 \pm 0.01$ \\
\sidehead{HCG 51}
A & $14.33 \pm 0.01$ & $13.51 \pm 0.01$ & $13.14 \pm 0.01$ \\
B & $14.89 \pm 0.01$ & $14.13 \pm 0.01$ & $13.78 \pm 0.01$ \\
C & $14.22 \pm 0.01$ & $13.41 \pm 0.01$ & $13.04 \pm 0.01$ \\
D & $15.47 \pm 0.01$ & $14.70 \pm 0.01$ & $14.37 \pm 0.01$ \\
E & $15.10 \pm 0.01$ & $14.25 \pm 0.01$ & $13.86 \pm 0.01$ \\
F & $15.80 \pm 0.01$ & $15.01 \pm 0.01$ & $14.67 \pm 0.01$ \\
G & $16.18 \pm 0.02$ & $15.36 \pm 0.02$ & $15.01 \pm 0.02$ \\
\sidehead{HCG 53}
A & $13.39 \pm 0.01$ & $12.78 \pm 0.01$ & $12.50 \pm 0.01$ \\
B & $14.51 \pm 0.01$ & $13.72 \pm 0.01$ & $13.37 \pm 0.01$ \\
C & $14.87 \pm 0.01$ & $14.43 \pm 0.01$ & $14.26 \pm 0.01$ \\
\sidehead{HCG 54}
A & $14.86 \pm 0.01$ & $14.59 \pm 0.01$ & $14.48 \pm 0.01$ \\
B & $16.34 \pm 0.02$ & $16.18 \pm 0.02$ & $16.26 \pm 0.03$ \\
C & $16.77 \pm 0.01$ & $16.68 \pm 0.01$ & $16.70 \pm 0.01$ \\
\sidehead{HCG 56}
A & $15.76 \pm 0.01$ & $15.02 \pm 0.01$ & $14.65 \pm 0.01$ \\
B & $14.51 \pm 0.01$ & $13.85 \pm 0.01$ & $13.58 \pm 0.01$ \\
C & $15.25 \pm 0.01$ & $14.51 \pm 0.01$ & $14.20 \pm 0.01$ \\
D & $16.11 \pm 0.01$ & $15.35 \pm 0.01$ & $15.00 \pm 0.01$ \\
E & $16.14 \pm 0.01$ & $15.61 \pm 0.01$ & $15.41 \pm 0.01$ \\
\sidehead{HCG 57\tablenotemark{f}}
A & $14.02 \pm 0.01$ & $13.16 \pm 0.01$ & $12.75 \pm 0.01$ \\
B & $14.39 \pm 0.01$ & $13.65 \pm 0.01$ & $13.33 \pm 0.01$ \\
C & $14.57 \pm 0.01$ & $13.77 \pm 0.01$ & $13.42 \pm 0.01$ \\
D & $15.05 \pm 0.01$ & $14.45 \pm 0.01$ & $14.21 \pm 0.01$ \\
E & $15.05 \pm 0.01$ & $14.23 \pm 0.01$ & $13.87 \pm 0.01$ \\
F & $15.19 \pm 0.01$ & $14.43 \pm 0.01$ & $14.11 \pm 0.01$ \\
G & $15.55 \pm 0.01$ & $14.74 \pm 0.01$ & $14.40 \pm 0.01$ \\
H & $16.66 \pm 0.01$ & $15.90 \pm 0.01$ & $15.60 \pm 0.01$ \\
\sidehead{HCG 58}
A & $13.41 \pm 0.01$ & $12.69 \pm 0.01$ & $12.38 \pm 0.01$ \\
B & $13.18 \pm 0.01$ & $12.44 \pm 0.01$ & $12.11 \pm 0.01$ \\
C & $13.78 \pm 0.01$ & $13.05 \pm 0.01$ & $12.72 \pm 0.01$ \\
D & $14.20 \pm 0.01$ & $13.41 \pm 0.01$ & $13.05 \pm 0.01$ \\
E & $14.80 \pm 0.01$ & $14.27 \pm 0.01$ & $14.05 \pm 0.01$ \\
\sidehead{HCG 59\tablenotemark{g}}
A & $14.39 \pm 0.01$ & $13.74 \pm 0.01$ & $13.47 \pm 0.01$ \\
B & $15.13 \pm 0.01$ & $14.42 \pm 0.01$ & $14.09 \pm 0.01$ \\
C & $15.76 \pm 0.01$ & $15.27 \pm 0.01$ & $15.06 \pm 0.01$ \\
D & $15.69 \pm 0.01$ & $15.46 \pm 0.01$ & $15.51 \pm 0.01$ \\
\sidehead{HCG 61\tablenotemark{h}}
A & $12.80 \pm 0.01$ & $12.03 \pm 0.01$ & $11.65 \pm 0.01$ \\
C & $13.86 \pm 0.01$ & $13.04 \pm 0.01$ & $12.63 \pm 0.01$ \\
D & $14.01 \pm 0.01$ & $13.33 \pm 0.01$ & $13.03 \pm 0.01$ \\
\sidehead{HCG 68\tablenotemark{i}}
D & $13.82 \pm 0.01$ & $13.16 \pm 0.01$ & $12.84 \pm 0.01$ \\
E & $14.26 \pm 0.01$ & $13.56 \pm 0.01$ & $13.22 \pm 0.01$ \\
\sidehead{HCG 69}
A & $14.98 \pm 0.01$ & $14.23 \pm 0.01$ & $13.85 \pm 0.01$ \\
B & $15.30 \pm 0.01$ & $14.63 \pm 0.01$ & $14.35 \pm 0.01$ \\
C & $15.57 \pm 0.01$ & $14.82 \pm 0.01$ & $14.51 \pm 0.01$ \\
D & $16.59 \pm 0.01$ & $15.81 \pm 0.01$ & $15.48 \pm 0.01$ \\
\sidehead{HCG 71}
A & $14.04 \pm 0.01$ & $13.39 \pm 0.01$ & $13.09 \pm 0.01$ \\
B & $15.03 \pm 0.01$ & $14.40 \pm 0.01$ & $14.13 \pm 0.01$ \\
C & $15.97 \pm 0.01$ & $15.51 \pm 0.01$ & $15.34 \pm 0.01$ \\
\sidehead{HCG 76}
A & $15.06 \pm 0.01$ & $14.22 \pm 0.01$ & $13.84 \pm 0.01$ \\
B & $14.73 \pm 0.01$ & $13.93 \pm 0.01$ & $13.57 \pm 0.01$ \\
C & $14.68 \pm 0.01$ & $13.88 \pm 0.01$ & $13.51 \pm 0.01$ \\
D & $15.11 \pm 0.01$ & $14.33 \pm 0.01$ & $13.98 \pm 0.01$ \\
E & $16.57 \pm 0.01$ & $15.82 \pm 0.01$ & $15.50 \pm 0.01$ \\
F & $16.58 \pm 0.01$ & $15.82 \pm 0.01$ & $15.48 \pm 0.01$ \\
G & $17.10 \pm 0.01$ & $16.32 \pm 0.01$ & $15.94 \pm 0.01$ \\
\sidehead{HCG 79\tablenotemark{j}}
A & $14.37 \pm 0.01$ & $13.57 \pm 0.01$ & $13.18 \pm 0.01$ \\
B & $13.99 \pm 0.01$ & $13.27 \pm 0.01$ & $12.93 \pm 0.01$ \\
C & $15.03 \pm 0.02$ & $14.38 \pm 0.02$ & $14.07 \pm 0.02$ \\
D & $15.87 \pm 0.01$ & $15.47 \pm 0.01$ & $15.30 \pm 0.01$ \\
\sidehead{HCG 88}
A & $13.48 \pm 0.02$ & $12.74 \pm 0.01$ & $12.38 \pm 0.01$ \\
B & $13.59 \pm 0.02$ & $12.88 \pm 0.01$ & $12.56 \pm 0.01$ \\
C & $14.33 \pm 0.02$ & $13.80 \pm 0.01$ & $13.59 \pm 0.01$ \\
D & $15.27 \pm 0.02$ & $14.70 \pm 0.01$ & $14.45 \pm 0.01$ \\
E\tablenotemark{\dag} & $17.88 \pm 0.02$ & $17.44 \pm 0.01$ & $17.30 \pm 0.01$ \\
\sidehead{HCG 89}
A & $14.86 \pm 0.02$ & $14.38 \pm 0.01$ & $14.22 \pm 0.01$ \\
B & $15.54 \pm 0.02$ & $15.11 \pm 0.01$ & $14.98 \pm 0.01$ \\
C & $16.06 \pm 0.02$ & $15.56 \pm 0.01$ & $15.38 \pm 0.01$ \\
D & $16.62 \pm 0.02$ & $16.39 \pm 0.01$ & $16.37 \pm 0.01$ \\
\sidehead{HCG 92\tablenotemark{k}}
B & $13.81 \pm 0.02$ & $13.10 \pm 0.02$ & $12.78 \pm 0.02$ \\
C & $13.65 \pm 0.02$ & $12.89 \pm 0.01$ & $12.57 \pm 0.01$ \\
D & $13.55 \pm 0.01$ & $12.81 \pm 0.01$ & $12.47 \pm 0.01$ \\
E & $14.37 \pm 0.01$ & $13.56 \pm 0.01$ & $13.17 \pm 0.01$ \\
\sidehead{HCG 93}
A & $12.49 \pm 0.03$ & $11.69 \pm 0.02$ & $11.31 \pm 0.02$ \\
B & $13.22 \pm 0.03$ & $12.62 \pm 0.02$ & $12.35 \pm 0.02$ \\
C & $13.76 \pm 0.03$ & $12.93 \pm 0.02$ & $12.56 \pm 0.02$ \\
D & $14.68 \pm 0.03$ & $13.84 \pm 0.02$ & $13.46 \pm 0.02$ \\
\sidehead{HCG 96}
A & $13.33 \pm 0.01$ & $12.82 \pm 0.01$ & $12.59 \pm 0.01$ \\
B & $14.17 \pm 0.01$ & $13.38 \pm 0.01$ & $13.04 \pm 0.01$ \\
C & $15.21 \pm 0.01$ & $14.49 \pm 0.01$ & $14.16 \pm 0.01$ \\
D & $16.62 \pm 0.01$ & $16.28 \pm 0.01$ & $16.18 \pm 0.01$ \\
\sidehead{HCG 97\tablenotemark{l}}
A & $13.71 \pm 0.01$ & $12.91 \pm 0.01$ & $12.54 \pm 0.01$ \\
B & $15.22 \pm 0.01$ & $14.49 \pm 0.01$ & $14.13 \pm 0.01$ \\
C & $14.41 \pm 0.01$ & $13.68 \pm 0.01$ & $13.35 \pm 0.01$ \\
D & $14.37 \pm 0.01$ & $13.55 \pm 0.01$ & $13.15 \pm 0.01$ \\
E & $16.08 \pm 0.01$ & $15.31 \pm 0.01$ & $14.96 \pm 0.01$ \\
\sidehead{HCG 98}
A & $13.54 \pm 0.01$ & $12.73 \pm 0.01$ & $12.35 \pm 0.01$ \\
B & $14.53 \pm 0.01$ & $13.72 \pm 0.01$ & $13.34 \pm 0.01$ \\
C & $15.83 \pm 0.01$ & $15.06 \pm 0.01$ & $14.72 \pm 0.01$ \\
\sidehead{HCG 99\tablenotemark{m}}
A & $14.22 \pm 0.01$ & $13.41 \pm 0.01$ & $12.98 \pm 0.01$ \\
B & $14.11 \pm 0.01$ & $13.30 \pm 0.01$ & $12.94 \pm 0.01$ \\
C & $14.99 \pm 0.01$ & $14.21 \pm 0.01$ & $13.86 \pm 0.01$ \\
D & $16.52 \pm 0.01$ & $15.75 \pm 0.01$ & $15.41 \pm 0.01$ \\
E & $16.94 \pm 0.01$ & $16.18 \pm 0.01$ & $15.84 \pm 0.01$ \\
\sidehead{HCG 100}
A & $13.41 \pm 0.01$ & $12.71 \pm 0.01$ & $12.41 \pm 0.01$ \\
B & $14.79 \pm 0.01$ & $14.38 \pm 0.01$ & $14.25 \pm 0.01$ \\
C & $15.34 \pm 0.01$ & $14.84 \pm 0.01$ & $14.64 \pm 0.01$ \\
D & $16.23 \pm 0.01$ & $15.77 \pm 0.01$ & $15.62 \pm 0.01$ \\
\enddata
\tablecomments{$^{\rm a}$RSCG 3. $^{\rm b}$RSCG 12. $^{\rm c}$RSCG 19. $^{\rm d}$RSCG 20. $^{\rm e}$RSCG 35. $^{\rm f}$RSCG 43. $^{\rm g}$RSCG 46. $^{\rm h}$RSCG 49. $^{\rm i}$RSCG 71. $^{\rm j}$RSCG 77. $^{\rm k}$RSCG 82. $^{\rm l}$RSCG 87. $^{\rm m}$RSCG 89. $^{\rm \dag}$Galaxy added by us.}
\end{deluxetable}

\endinput
%%
%% End of file `hcggals.tex'.


==> rscggals.tex <==
\ProvidesFile{rscggals.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{ccccc}
\tabletypesize{\small}
\tablewidth{0pt}
\tablecolumns{5}
\tablecaption{Photometry for RSCG Galaxies\label{rscggals}}
\tablehead{
\multicolumn{2}{c}{Galaxy} &	\colhead{g'} &	\colhead{r'} &	\colhead{i'} \\
\colhead{} &	\colhead{} &	\colhead{mag} &	\colhead{mag} &	\colhead{mag}
}
\startdata
\sidehead{RSCG 1}
A & NGC 70 & $13.04 \pm 0.02$ & $12.33 \pm 0.02$ & $11.99 \pm 0.01$ \\
B & NGC 68 & $13.76 \pm 0.02$ & $12.96 \pm 0.01$ & $12.60 \pm 0.01$ \\
C & NGC 71 & $13.93 \pm 0.02$ & $13.14 \pm 0.02$ & $12.77 \pm 0.01$ \\
D & NGC 72 & $14.10 \pm 0.02$ & $13.28 \pm 0.01$ & $12.92 \pm 0.01$ \\
E & NGC 72A & $15.25 \pm 0.02$ & $14.44 \pm 0.01$ & $14.08 \pm 0.01$ \\
\sidehead{RSCG 2}
A & UGC 335b & $14.22 \pm 0.01$ & $13.45 \pm 0.01$ & $13.09 \pm 0.01$ \\
B & UGC 335a & $14.62 \pm 0.01$ & $13.83 \pm 0.01$ & $13.48 \pm 0.01$ \\
C & UGC 331 & $15.00 \pm 0.01$ & $14.28 \pm 0.01$ & $13.98 \pm 0.01$ \\
\sidehead{RSCG 4}
A & NGC 235B & $13.69 \pm 0.01$ & $12.97 \pm 0.01$ & $12.65 \pm 0.01$ \\
B & NGC 235A & $15.21 \pm 0.01$ & $14.47 \pm 0.01$ & $14.14 \pm 0.01$ \\
C & NGC 232 & \nodata & \nodata & \nodata\\
\sidehead{RSCG 5}
A & NGC 383 & $12.58 \pm 0.02$ & $11.76 \pm 0.02$ & $11.34 \pm 0.01$ \\
B & NGC 385 & $13.58 \pm 0.02$ & $12.79 \pm 0.01$ & $12.42 \pm 0.01$ \\
C & NGC 384 & $13.74 \pm 0.02$ & $12.95 \pm 0.01$ & $12.55 \pm 0.01$ \\
D & NGC 382 & $13.94 \pm 0.02$ & $13.13 \pm 0.02$ & $12.73 \pm 0.02$ \\
E & NGC 386 & $14.85 \pm 0.02$ & $14.09 \pm 0.01$ & $13.73 \pm 0.01$ \\
\sidehead{RSCG 6}
A & UGC 816 & $13.87 \pm 0.01$ & $13.37 \pm 0.01$ & $13.22 \pm 0.01$ \\
B & UGC 813 & $14.21 \pm 0.01$ & $13.68 \pm 0.01$ & $13.46 \pm 0.01$ \\
C & CGCG 551-011 & $14.43 \pm 0.01$ & $13.71 \pm 0.01$ & $13.38 \pm 0.01$ \\
\sidehead{RSCG 7}
A & NGC 499 & $12.64 \pm 0.01$ & $11.81 \pm 0.01$ & $11.41 \pm 0.01$ \\
B & NGC 495 & $13.62 \pm 0.01$ & $12.82 \pm 0.01$ & $12.45 \pm 0.01$ \\
C & NGC 501 & $14.83 \pm 0.01$ & $14.03 \pm 0.01$ & $13.65 \pm 0.01$ \\
\sidehead{RSCG 8}
A & NGC 507 & $12.04 \pm 0.01$ & $11.23 \pm 0.01$ & $10.83 \pm 0.01$ \\
C & NGC 508 & $13.93 \pm 0.01$ & $13.05 \pm 0.01$ & $12.63 \pm 0.01$ \\
B & NGC 504 & $13.82 \pm 0.01$ & $13.01 \pm 0.01$ & $12.64 \pm 0.01$ \\
D & IC 1687 & $14.66 \pm 0.01$ & $13.85 \pm 0.01$ & $13.48 \pm 0.01$ \\
E & NGC 503 & $14.75 \pm 0.01$ & $13.97 \pm 0.01$ & $13.62 \pm 0.01$ \\
\sidehead{RSCG 9}
A & UGC 978 & $13.60 \pm 0.01$ & $12.82 \pm 0.01$ & $12.46 \pm 0.01$ \\
B & IC 107 & $14.29 \pm 0.01$ & $13.53 \pm 0.01$ & $13.20 \pm 0.01$ \\
C & IC 1698 & $14.68 \pm 0.01$ & $14.18 \pm 0.01$ & $14.00 \pm 0.01$ \\
\sidehead{RSCG 10}
A & NGC 538 & $13.86 \pm 0.01$ & $13.05 \pm 0.01$ & $12.65 \pm 0.01$ \\
B & UGC 996 & $14.40 \pm 0.01$ & $13.64 \pm 0.01$ & $13.30 \pm 0.01$ \\
C & UGC 984 & $14.43 \pm 0.01$ & $13.70 \pm 0.01$ & $13.36 \pm 0.01$ \\
\sidehead{RSCG 11}
A/B & NGC 547/545 & $11.98 \pm 0.01$ & $11.18 \pm 0.01$ & $10.79 \pm 0.01$ \\
%B & NGC 545 & $ \pm $ & $ &$\\
C & NGC 541 & $12.99 \pm 0.01$ & $12.21 \pm 0.01$ & $11.83 \pm 0.01$ \\
D & NGC 543 & $14.47 \pm 0.01$ & $13.66 \pm 0.01$ & $13.28 \pm 0.01$ \\
E & ARK 45 & $14.87 \pm 0.01$ & $14.08 \pm 0.01$ & $13.71 \pm 0.01$ \\
\sidehead{RSCG 14}
A & NGC 680 & $12.18 \pm 0.02$ & $11.41 \pm 0.01$ & $11.04 \pm 0.01$ \\
B & NGC 678 & $12.56 \pm 0.02$ & $11.66 \pm 0.01$ & $11.20 \pm 0.01$ \\
C & IC 1730 & $14.85 \pm 0.02$ & $14.18 \pm 0.01$ & $13.87 \pm 0.01$ \\
\sidehead{RSCG 17}
A & NGC 741 & $12.15 \pm 0.01$ & $11.32 \pm 0.01$ & $10.92 \pm 0.01$ \\
B & ARK 66 & $14.09 \pm 0.02$ & $13.25 \pm 0.02$ & $12.84 \pm 0.01$ \\
C & NGC 742 & $14.88 \pm 0.01$ & $14.05 \pm 0.01$ & $13.68 \pm 0.01$ \\
\sidehead{RSCG 18}
A & NGC 736 & $12.77 \pm 0.01$ & $11.97 \pm 0.01$ & $11.58 \pm 0.01$ \\
B & NGC 740 & $14.40 \pm 0.01$ & $13.70 \pm 0.01$ & $13.37 \pm 0.01$ \\
C & NGC 738 & $15.22 \pm 0.01$ & $14.44 \pm 0.01$ & $14.09 \pm 0.01$ \\
\sidehead{RSCG 21}
A & NGC 1273 & $13.47 \pm 0.02$ & $12.70 \pm 0.01$ & $12.37 \pm 0.01$ \\
B & NGC 1277 & $13.83 \pm 0.02$ & $12.99 \pm 0.01$ & $12.60 \pm 0.01$ \\
C & CGCG 540-101 & $13.84 \pm 0.02$ & $13.00 \pm 0.01$ & $12.61 \pm 0.01$ \\
\sidehead{RSCG 28}
A & NGC 2738 & $13.37 \pm 0.01$ & $12.87 \pm 0.01$ & $12.63 \pm 0.01$ \\
B & NGC 2737 & $13.86 \pm 0.01$ & $13.14 \pm 0.01$ & $12.79 \pm 0.01$ \\
C & CGCG 121-011 & $15.09 \pm 0.01$ & $14.73 \pm 0.01$ & $14.58 \pm 0.01$ \\
\sidehead{RSCG 30}
A & NGC 2778 & $13.06 \pm 0.01$ & $12.31 \pm 0.01$ & $11.93 \pm 0.01$ \\
B & NGC 2780 & $13.98 \pm 0.01$ & $13.36 \pm 0.01$ & $13.06 \pm 0.01$ \\
C & NGC 2779 & $15.12 \pm 0.01$ & $14.50 \pm 0.01$ & $14.23 \pm 0.01$ \\
\sidehead{RSCG 31}
A & NGC 2798 & $12.70 \pm 0.01$ & $12.00 \pm 0.01$ & $11.70 \pm 0.01$ \\
B & NGC 2799 & $13.94 \pm 0.01$ & $13.47 \pm 0.01$ & $13.28 \pm 0.01$ \\
C & UGC 4904 & $14.56 \pm 0.01$ & $14.17 \pm 0.01$ & $14.01 \pm 0.01$ \\
\sidehead{RSCG 32}
A & NGC 2832 & $12.40 \pm 0.01$ & $11.57 \pm 0.01$ & $11.17 \pm 0.01$ \\
B & NGC 2831 & $14.28 \pm 0.02$ & $13.46 \pm 0.02$ & $13.07 \pm 0.02$ \\
C & NGC 2830 & $14.56 \pm 0.01$ & $13.80 \pm 0.01$ & $13.45 \pm 0.01$ \\
\sidehead{RSCG 33}
A & NGC 2911 & $12.40 \pm 0.01$ & $11.56 \pm 0.01$ & $11.14 \pm 0.01$ \\
B & NGC 2914 & $13.52 \pm 0.01$ & $12.76 \pm 0.01$ & $12.38 \pm 0.01$ \\
C & UGC 5093 & $14.72 \pm 0.01$ & $14.05 \pm 0.01$ & $13.72 \pm 0.01$ \\
\sidehead{RSCG 34}
A & NGC 2964 & $11.64 \pm 0.01$ & $11.05 \pm 0.01$ & $10.77 \pm 0.01$ \\
B & NGC 2968 & $12.32 \pm 0.01$ & $11.42 \pm 0.01$ & $10.94 \pm 0.01$ \\
C & NGC 2970 & $14.25 \pm 0.01$ & $13.67 \pm 0.01$ & $13.38 \pm 0.01$ \\
\sidehead{RSCG 36}
A & NGC 3379 & $9.92 \pm 0.01$ & $9.16 \pm 0.01$ & $8.76 \pm 0.01$ \\
B & NGC 3384 & $10.38 \pm 0.01$ & $9.64 \pm 0.01$ & $9.27 \pm 0.01$ \\
C & NGC 3389 & $12.03 \pm 0.01$ & $11.69 \pm 0.01$ & $11.53 \pm 0.01$ \\
\sidehead{RSCG 37}
A & NGC 3377 & $10.84 \pm 0.01$ & $10.16 \pm 0.01$ & $9.83 \pm 0.01$ \\
B & NGC 3377A & $14.04 \pm 0.01$ & $13.58 \pm 0.01$ & $13.35 \pm 0.01$ \\
C & CGCG 066-026 & $15.57 \pm 0.01$ & $14.96 \pm 0.01$ & $14.66 \pm 0.01$ \\
\sidehead{RSCG 38}
A & NGC 3430 & $11.89 \pm 0.01$ & $11.39 \pm 0.01$ & $11.17 \pm 0.01$ \\
B & NGC 3424 & $12.81 \pm 0.01$ & $12.13 \pm 0.01$ & $11.77 \pm 0.01$ \\
C & NGC 3413 & $13.05 \pm 0.01$ & $12.70 \pm 0.01$ & $12.54 \pm 0.01$ \\
\sidehead{RSCG 39}
A & NGC 3455 & $12.91 \pm 0.01$ & $12.57 \pm 0.01$ & $12.41 \pm 0.01$ \\
B & NGC 3454 & $13.69 \pm 0.01$ & $13.11 \pm 0.01$ & $12.83 \pm 0.01$ \\
C & UGC 6035 & $14.57 \pm 0.01$ & $14.23 \pm 0.01$ & $14.05 \pm 0.01$ \\
D & CGCG 095-070 & $15.20 \pm 0.01$ & $14.80 \pm 0.01$ & $14.61 \pm 0.01$ \\
\sidehead{RSCG 40}
A & NGC 3607 & $10.54 \pm 0.01$ & $9.79 \pm 0.01$ & $9.39 \pm 0.01$ \\
B & NGC 3608 & $11.57 \pm 0.01$ & $10.82 \pm 0.01$ & $10.44 \pm 0.01$ \\
C & NGC 3599 & $12.49 \pm 0.01$ & $11.83 \pm 0.01$ & $11.47 \pm 0.01$ \\
D & NGC 3605 & $13.12 \pm 0.01$ & $12.42 \pm 0.01$ & $12.06 \pm 0.01$ \\
E & UGC 6296 & $13.97 \pm 0.01$ & $13.31 \pm 0.01$ & $12.96 \pm 0.01$ \\
\sidehead{RSCG 41}
A & NGC 3686 & $11.55 \pm 0.01$ & $11.03 \pm 0.01$ & $10.76 \pm 0.01$ \\
B & NGC 3684 & $12.12 \pm 0.01$ & $11.65 \pm 0.01$ & $11.28 \pm 0.02$ \\
C & NGC 3681 & $12.16 \pm 0.01$ & $11.53 \pm 0.01$ & $11.20 \pm 0.01$ \\
D & NGC 3691 & $13.20 \pm 0.01$ & $12.77 \pm 0.01$ & $12.58 \pm 0.01$ \\
\sidehead{RSCG 42}
A & UGC 6583 & $14.09 \pm 0.01$ & $13.65 \pm 0.01$ & $13.51 \pm 0.01$ \\
B & KUG 1134+202A & $14.53 \pm 0.01$ & $13.96 \pm 0.01$ & $13.71 \pm 0.01$ \\
C & ARK 303 & $14.98 \pm 0.01$ & $14.23 \pm 0.01$ & $13.89 \pm 0.01$ \\
\sidehead{RSCG 44}
A & NGC 3842 & $12.67 \pm 0.01$ & $11.87 \pm 0.01$ & $11.48 \pm 0.01$ \\
B & NGC 3837 & $13.74 \pm 0.01$ & $12.93 \pm 0.01$ & $12.55 \pm 0.01$ \\
C & UGC 6697 & $13.81 \pm 0.01$ & $13.43 \pm 0.01$ & $13.28 \pm 0.01$ \\
D & NGC 3841 & $14.30 \pm 0.01$ & $13.49 \pm 0.01$ & $13.14 \pm 0.01$ \\
E & NGC 3845 & $14.71 \pm 0.01$ & $13.96 \pm 0.01$ & $13.62 \pm 0.01$ \\
\sidehead{RSCG 45}
A & CGCG 97-101 & $14.52 \pm 0.01$ & $13.73 \pm 0.01$ & $13.35 \pm 0.01$ \\
B & CGCG 97-105 & $14.98 \pm 0.01$ & $14.19 \pm 0.01$ & $13.84 \pm 0.01$ \\
C & CGCG 97-110 & $15.21 \pm 0.01$ & $14.47 \pm 0.01$ & $14.12 \pm 0.01$ \\
\sidehead{RSCG 47}
A & NGC 3995 & $12.50 \pm 0.01$ & $12.27 \pm 0.01$ & $12.23 \pm 0.01$ \\
B & NGC 3994 & $13.10 \pm 0.01$ & $12.49 \pm 0.01$ & $12.22 \pm 0.01$ \\
C & NGC 3991N & $13.98 \pm 0.01$ & $13.88 \pm 0.01$ & $13.98 \pm 0.01$ \\
D & NGC 3991S & $14.13 \pm 0.01$ & $13.73 \pm 0.01$ & $13.59 \pm 0.01$ \\
\sidehead{RSCG 48}
A & NGC 4111 & $11.05 \pm 0.01$ & $10.44 \pm 0.01$ & $9.97 \pm 0.01$ \\
B & NGC 4117 & $13.43 \pm 0.01$ & $12.70 \pm 0.01$ & $12.33 \pm 0.01$ \\
C & UGC 7089 & $13.47 \pm 0.01$ & $13.06 \pm 0.01$ & $12.83 \pm 0.01$ \\
\sidehead{RSCG 50}
A & NGC 4206 & $12.55 \pm 0.01$ & $12.00 \pm 0.01$ & $11.70 \pm 0.01$ \\
B & IC 3056 & $15.26 \pm 0.01$ & $14.94 \pm 0.01$ & $14.83 \pm 0.01$ \\
C & IC 3066 & $15.34 \pm 0.01$ & $14.85 \pm 0.01$ & $14.60 \pm 0.01$ \\
\sidehead{RSCG 51}
A & NGC 4274 & $10.89 \pm 0.01$ & $10.09 \pm 0.01$ & $9.67 \pm 0.01$ \\
B & NGC 4278 & $10.71 \pm 0.01$ & $9.95 \pm 0.01$ & $9.53 \pm 0.01$ \\
C & NGC 4314 & $10.93 \pm 0.01$ & $10.20 \pm 0.01$ & $9.82 \pm 0.01$ \\
D & NGC 4283 & $12.71 \pm 0.01$ & $11.96 \pm 0.01$ & $11.56 \pm 0.01$ \\
E & NGC 4286 & $13.93 \pm 0.01$ & $13.33 \pm 0.01$ & $13.02 \pm 0.01$ \\
F & NGC 4308 & $13.96 \pm 0.01$ & $13.29 \pm 0.01$ & $12.95 \pm 0.01$ \\
G & IC 779 & $14.83 \pm 0.01$ & $14.20 \pm 0.01$ & $13.89 \pm 0.01$ \\
H & SDSS J122120.10+294255.7 & $15.89 \pm 0.01$ & $15.27 \pm 0.01$ & $14.97 \pm 0.01$ \\
I & SDSS J121943.54+293931.7 & $17.70 \pm 0.02$ & $17.09 \pm 0.02$ & $16.81 \pm 0.02$ \\
\sidehead{RSCG 52}
A & CGCG 215-065 & $14.49 \pm 0.01$ & $13.75 \pm 0.01$ & $13.42 \pm 0.01$ \\
B & KUG 1218+401A & $14.68 \pm 0.01$ & $14.19 \pm 0.01$ & $14.02 \pm 0.01$ \\
C & KUG 1218+401B & $14.80 \pm 0.01$ & $14.38 \pm 0.01$ & $14.25 \pm 0.01$ \\
\sidehead{RSCG 53}
A & NGC 4298 & $11.61 \pm 0.01$ & $10.98 \pm 0.01$ & $10.66 \pm 0.01$ \\
B & NGC 4302 & $11.93 \pm 0.01$ & $11.13 \pm 0.01$ & $10.67 \pm 0.01$ \\
C & UGC 7436 & $14.15 \pm 0.01$ & $13.50 \pm 0.01$ & $13.19 \pm 0.01$ \\
\sidehead{RSCG 54}
A & NGC 4382 & $9.48 \pm 0.01$ & $8.81 \pm 0.01$ & $8.41 \pm 0.01$ \\
B & NGC 4394 & $11.37 \pm 0.01$ & $10.70 \pm 0.01$ & $10.36 \pm 0.01$ \\
C & IC 3292 & $14.65 \pm 0.01$ & $13.97 \pm 0.01$ & $13.61 \pm 0.01$ \\
\sidehead{RSCG 55}
A & NGC 4410B & $13.78 \pm 0.01$ & $12.97 \pm 0.01$ & $12.58 \pm 0.01$ \\
B & NGC 4410A & $13.85 \pm 0.01$ & $13.06 \pm 0.01$ & $12.71 \pm 0.01$ \\
C & NGC 4410C & $14.63 \pm 0.01$ & $13.78 \pm 0.01$ & $13.40 \pm 0.01$ \\
D & NGC 4410D & $15.20 \pm 0.01$ & $14.55 \pm 0.01$ & $14.29 \pm 0.01$ \\
E & NGC 4410F & $16.63 \pm 0.01$ & $16.26 \pm 0.01$ & $16.18 \pm 0.01$ \\
\sidehead{RSCG 56}
A & NGC 4440 & $12.31 \pm 0.01$ & $11.58 \pm 0.01$ & $11.23 \pm 0.01$ \\
B & NGC 4431 & $13.62 \pm 0.01$ & $12.92 \pm 0.01$ & $12.58 \pm 0.01$ \\
C & NGC 4436 & $13.76 \pm 0.01$ & $13.09 \pm 0.01$ & $12.76 \pm 0.01$ \\
D & IC 3349 & $14.78 \pm 0.01$ & $14.10 \pm 0.01$ & $13.79 \pm 0.01$ \\
E & IC 3363 & $15.20 \pm 0.01$ & $14.60 \pm 0.01$ & $14.30 \pm 0.01$ \\
\sidehead{RSCG 57}
A & NGC 4442 & $10.94 \pm 0.01$ & $10.18 \pm 0.01$ & $9.79 \pm 0.01$ \\
B & NGC 4417 & $11.66 \pm 0.01$ & $10.92 \pm 0.01$ & $10.54 \pm 0.01$ \\
C & NGC 4424 & $11.94 \pm 0.01$ & $11.39 \pm 0.01$ & $11.09 \pm 0.01$ \\
D & NGC 4451 & $12.97 \pm 0.01$ & $12.39 \pm 0.01$ & $12.10 \pm 0.01$ \\
E & NGC 4445 & $13.20 \pm 0.01$ & $12.49 \pm 0.01$ & $12.12 \pm 0.01$ \\
F & IC 3412 & $15.39 \pm 0.01$ & $15.00 \pm 0.01$ & $14.82 \pm 0.01$ \\
G & VCC 1078 & $15.82 \pm 0.01$ & $15.42 \pm 0.01$ & $15.23 \pm 0.01$ \\
\sidehead{RSCG 58}
A & NGC 4435 & $11.20 \pm 0.01$ & $10.44 \pm 0.01$ & $10.05 \pm 0.01$ \\
B & NGC 4458 & $12.66 \pm 0.01$ & $11.97 \pm 0.01$ & $11.59 \pm 0.01$ \\
C & IC 3393 & $14.76 \pm 0.01$ & $14.15 \pm 0.01$ & $13.86 \pm 0.01$ \\
\sidehead{RSCG 59}
A & NGC 4459 & $11.29 \pm 0.02$ & $10.50 \pm 0.01$ & $10.10 \pm 0.01$ \\
B & NGC 4474 & $12.35 \pm 0.01$ & $11.64 \pm 0.01$ & $11.27 \pm 0.01$ \\
C & NGC 4468 & $13.57 \pm 0.01$ & $12.89 \pm 0.01$ & $12.54 \pm 0.01$ \\
\sidehead{RSCG 60}
A & NGC 4469 & $11.62 \pm 0.01$ & $10.87 \pm 0.01$ & $10.47 \pm 0.01$ \\
B & NGC 4483 & $12.77 \pm 0.01$ & $12.03 \pm 0.01$ & $11.66 \pm 0.01$ \\
C & UGC 7590 & $14.00 \pm 0.01$ & $13.71 \pm 0.01$ & $13.54 \pm 0.01$ \\
D\tablenotemark{\dag} & UGC 7596 & $14.74 \pm 0.01$ & $14.31 \pm 0.01$ & $14.09 \pm 0.01$ \\
\sidehead{RSCG 61}
A & M 87 & $9.99 \pm 0.01$ & $9.19 \pm 0.01$ & $8.78 \pm 0.01$ \\
B & NGC 4478 & $11.84 \pm 0.01$ & $11.12 \pm 0.01$ & $10.75 \pm 0.01$ \\
C & NGC 4486A & $12.46 \pm 0.01$ & $11.91 \pm 0.01$ & $11.56 \pm 0.01$ \\
D & NGC 4486B & $13.83 \pm 0.01$ & $13.03 \pm 0.01$ & $12.64 \pm 0.01$ \\
\sidehead{RSCG 62}
A & NGC 4497 & $12.84 \pm 0.02$ & $12.17 \pm 0.02$ & $11.85 \pm 0.01$ \\
B & NGC 4491 & $13.00 \pm 0.02$ & $12.37 \pm 0.02$ & $12.04 \pm 0.01$ \\
C & IC 3461 & $15.03 \pm 0.02$ & $14.39 \pm 0.02$ & $14.07 \pm 0.01$ \\
D & IC 3466 & $15.15 \pm 0.02$ & $14.81 \pm 0.02$ & $14.68 \pm 0.01$ \\
E & IC 3446 & $15.54 \pm 0.02$ & $15.19 \pm 0.02$ & $15.02 \pm 0.02$ \\
\sidehead{RSCG 63}
A & NGC 4552 & $10.90 \pm 0.01$ & $10.11 \pm 0.01$ & $9.72 \pm 0.01$ \\
B & NGC 4550 & $12.06 \pm 0.01$ & $11.34 \pm 0.01$ & $10.99 \pm 0.01$ \\
C & NGC 4551 & $12.63 \pm 0.01$ & $11.87 \pm 0.01$ & $11.49 \pm 0.01$ \\
D & IC 3540 & $14.26 \pm 0.01$ & $13.68 \pm 0.01$ & $13.40 \pm 0.01$ \\
\sidehead{RSCG 64}
A & NGC 4615 & $13.56 \pm 0.01$ & $13.14 \pm 0.01$ & $12.99 \pm 0.01$ \\
B & NGC 4614 & $13.83 \pm 0.01$ & $13.12 \pm 0.01$ & $12.80 \pm 0.01$ \\
C & NGC 4613 & $15.09 \pm 0.01$ & $14.43 \pm 0.01$ & $14.14 \pm 0.01$ \\
\sidehead{RSCG 65}
A & NGC 4649 & $9.93 \pm 0.01$ & $9.12 \pm 0.01$ & $8.69 \pm 0.01$ \\
B & NGC 4621 & $10.77 \pm 0.01$ & $9.98 \pm 0.01$ & $9.56 \pm 0.01$ \\
C & NGC 4647 & $11.51 \pm 0.01$ & $10.91 \pm 0.01$ & $10.60 \pm 0.01$ \\
D & NGC 4638 & $11.70 \pm 0.01$ & $10.97 \pm 0.01$ & $10.60 \pm 0.01$ \\
E & IC 3653 & $14.09 \pm 0.01$ & $13.35 \pm 0.01$ & $12.99 \pm 0.01$ \\
F & IC 3652 & $14.18 \pm 0.01$ & $13.52 \pm 0.01$ & $13.18 \pm 0.01$ \\
G & IC 3665 & $14.99 \pm 0.01$ & $14.44 \pm 0.01$ & $14.17 \pm 0.01$ \\
\sidehead{RSCG 66}
A & NGC 4654 & $10.81 \pm 0.01$ & $10.30 \pm 0.01$ & $10.04 \pm 0.01$ \\
B & NGC 4639 & $11.86 \pm 0.01$ & $11.27 \pm 0.01$ & $10.96 \pm 0.01$ \\
C & VCC 1931 & $15.74 \pm 0.01$ & $15.47 \pm 0.01$ & $15.35 \pm 0.01$ \\
\sidehead{RSCG 67**}
A & NGC 4874 & $12.55 \pm 0.01$ & $11.73 \pm 0.01$ & $11.33 \pm 0.01$ \\
B & NGC 4871 & $14.75 \pm 0.01$ & $13.94 \pm 0.01$ & $13.59 \pm 0.01$ \\
C & NGC 4872 & $14.91 \pm 0.02$ & $14.10 \pm 0.02$ & $13.74 \pm 0.02$ \\
\sidehead{RSCG 68**}
A & NGC 4889 & $13.02 \pm 0.01$ & $12.18 \pm 0.01$ & $11.79 \pm 0.01$ \\
B & NGC 4898W & $14.26 \pm 0.01$ & $13.47 \pm 0.01$ & $13.11 \pm 0.01$ \\
C & NGC 4886 & $14.63 \pm 0.01$ & $13.87 \pm 0.01$ & $13.50 \pm 0.01$ \\
\sidehead{RSCG 69}
A & IC 867 & $14.28 \pm 0.01$ & $13.67 \pm 0.01$ & $13.39 \pm 0.01$ \\
B & IC 868 & $14.39 \pm 0.01$ & $13.59 \pm 0.01$ & $13.24 \pm 0.01$ \\
C & IC 870 & $14.53 \pm 0.01$ & $13.93 \pm 0.01$ & $13.68 \pm 0.01$ \\
\sidehead{RSCG 72}
A & IC 962 & $13.70 \pm 0.01$ & $13.04 \pm 0.01$ & $12.75 \pm 0.01$ \\
B & CGCG 74-014 & $14.75 \pm 0.01$ & $14.06 \pm 0.01$ & $13.74 \pm 0.01$ \\
C & CGCG 74-016 & $15.20 \pm 0.01$ & $14.81 \pm 0.01$ & $14.66 \pm 0.01$ \\
\sidehead{RSCG 73}
A & NGC 5423 & $13.43 \pm 0.01$ & $12.63 \pm 0.01$ & $12.26 \pm 0.01$ \\
B & CGCG 074-058 & $14.96 \pm 0.01$ & $14.18 \pm 0.01$ & $13.83 \pm 0.01$ \\
C & CGCG 074-062 & $15.56 \pm 0.01$ & $14.85 \pm 0.01$ & $14.53 \pm 0.01$ \\
\sidehead{RSCG 74}
A & NGC 5504 & $13.50 \pm 0.01$ & $12.98 \pm 0.01$ & $12.75 \pm 0.01$ \\
B & NGC 5504B & $15.06 \pm 0.01$ & $14.49 \pm 0.01$ & $14.25 \pm 0.01$ \\
C & NGC 5504C & $15.59 \pm 0.01$ & $15.36 \pm 0.01$ & $15.29 \pm 0.01$ \\
\sidehead{RSCG 75}
A & UGC 9521 & $13.99 \pm 0.01$ & $13.25 \pm 0.01$ & $12.90 \pm 0.01$ \\
B & UGC 9523 & $14.08 \pm 0.01$ & $13.28 \pm 0.01$ & $12.92 \pm 0.01$ \\
C & CGCG 76-040 & $15.14 \pm 0.01$ & $14.35 \pm 0.01$ & $14.00 \pm 0.01$ \\
\sidehead{RSCG 76}
A & NGC 5852 & $13.86 \pm 0.01$ & $13.03 \pm 0.01$ & $12.64 \pm 0.01$ \\
B & NGC 5851 & $14.42 \pm 0.01$ & $13.78 \pm 0.01$ & $13.50 \pm 0.01$ \\
C & CGCG 77-007 & $15.51 \pm 0.01$ & $14.90 \pm 0.01$ & $14.63 \pm 0.01$ \\
\sidehead{RSCG 78}
A & NGC 6962 & $12.07 \pm 0.02$ & $11.36 \pm 0.01$ & $11.01 \pm 0.01$ \\
B & NGC 6964 & $13.19 \pm 0.02$ & $12.41 \pm 0.01$ & $12.04 \pm 0.01$ \\
C & NGC 6959 & $13.89 \pm 0.02$ & $13.21 \pm 0.01$ & $12.93 \pm 0.01$ \\
D & NGC 6961 & $14.60 \pm 0.02$ & $13.82 \pm 0.01$ & $13.46 \pm 0.01$ \\
\sidehead{RSCG 83}
A & NGC 7463 & $12.87 \pm 0.02$ & $12.48 \pm 0.01$ & $12.30 \pm 0.01$ \\
B & NGC 7465 & $12.87 \pm 0.02$ & $12.25 \pm 0.01$ & $11.98 \pm 0.01$ \\
C & NGC 7464 & $14.37 \pm 0.02$ & $14.22 \pm 0.01$ & $14.20 \pm 0.01$ \\
\sidehead{RSCG 84}
A & NGC 7532 & $13.86 \pm 0.01$ & $13.42 \pm 0.01$ & $13.24 \pm 0.01$ \\
B & NGC 7534 & $14.29 \pm 0.01$ & $14.04 \pm 0.01$ & $13.98 \pm 0.01$ \\
C & NGC 7533 & $14.62 \pm 0.01$ & $14.16 \pm 0.01$ & $13.97 \pm 0.01$ \\
\sidehead{RSCG 85}
A & UGC 12545 & $14.59 \pm 0.02$ & $14.15 \pm 0.01$ & $13.99 \pm 0.01$ \\
B & UGC 12546 & $14.62 \pm 0.02$ & $14.06 \pm 0.01$ & $13.83 \pm 0.01$ \\
C & UGC 12543 & $15.18 \pm 0.02$ & $14.71 \pm 0.01$ & $14.50 \pm 0.01$ \\
\sidehead{RSCG 86}
A & UGC 12716a & $13.28 \pm 0.02$ & $12.43 \pm 0.02$ & $12.04 \pm 0.01$ \\
B & IC 5342 & $14.85 \pm 0.02$ & $14.03 \pm 0.01$ & $13.66 \pm 0.01$ \\
C & UGC 12716b & $15.00 \pm 0.02$ & $14.16 \pm 0.02$ & $13.78 \pm 0.02$ \\
D & 2MASX J23383626+2701467 & $15.31 \pm 0.02$ & $14.46 \pm 0.01$ & $14.07 \pm 0.01$ \\
\enddata
\tablecomments{$^{\rm \dag}$Galaxy added by us. **Groups embedded in Perseus (RSCG 21) or Coma (RSCGs 67 \& 68). These were excluded from our analysis.}
\end{deluxetable}

\endinput
%%
%% End of file `rscggals.tex'.

